The Value of Summary Statistics for Anomaly Detection in Temporally-Evolving Networks: A Performance Evaluation Study

Network data has emerged as an active research area in statistics. Much of the focus of ongoing research has been on static networks that represent a single snapshot or aggregated historical data unchanging over time. However, most networks result from temporally-evolving systems that exhibit intrinsic dynamic behavior. Monitoring such temporally-varying networks to detect anomalous changes has applications in both social and physical sciences. In this work, we perform an evaluation study of summary statistics for anomaly detection in temporally-evolving networks by incorporating principles from statistical process monitoring. In contrast to previous studies, we deliberately incorporate temporal auto-correlation in our study. Other considerations in our comprehensive assessment include types and duration of anomaly, model type, and sparsity in temporally-evolving networks. We conclude that summary statistics can be valuable tools for network monitoring and often perform better than more complicated statistics.

==> Sec5DataApp.tex <==
\section{Applications} \label{sec:application}
%-----------------------------------------------
%-----------------------------------------------

\uhoh{Need to flesh this out better or find another application.}

Our methods are applied to MIT Reality Mining Data \citep{eagle2006reality}. The particular data we use consists of 10 minute intervals for approximately 210 days of 96 individuals (27 faculty and 69 students). An edge in this network indicates person A and B were within 5 meters of proximity of each other recorded via cell phone communication logs \citep{eagle2009inferring}. Data was collected from September 2004 until April 2005. In Figure \ref{fig:MIT_Dens}, we observe network density over the course of 30 weeks (Fall and Spring semesters). We notice much more activity in Fall than Spring semesters, and the larger gap after 100 days is presumed to be winter break. 

% MIT DENSITY OVERALL
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\begin{figure}[H]
\centering
\includegraphics[width=2.65in,angle=270]{IMG/MIT_1.eps}
\caption{Network Density of MIT Reality Mining Data.} 
\label{fig:MIT_Dens}
\end{figure}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

Next, weekday and weekend activity is compared hourly in Figure \ref{fig:MIT_Hrly}. Each day is overlaid on the same plot organized by weekday or weekend. We observe weekends have much less activity than weekdays, and for weekdays, there is a lull in activity between hours 8 to 14 while for weekends, the lull period is between hours 10 to 18.

% MIT DENSITY WEEKDAY VS WEEKEND
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\begin{figure}[H]
\centering
\includegraphics[width=4in,angle=270]{IMG/MIT_2.eps}
\caption{Hourly Weekday and Weekend Network Density of MIT Reality Mining Data.} 
\label{fig:MIT_Hrly}
\end{figure}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

% We calculate $M_t$ using hours 8 to 14 as an inactive period and the remaining 17 hours as an active period for weekdays and weekends separately.

We first apply our methods for each hour of each day. In Figure \ref{fig:MIT_Mt}, we calculate a mean and standard deviation using the first 5 weeks as Phase I data. The mean of Phase I data is indicated using a blue solid line and the dashed mustard yellow line indicates $\overline{x} + 2 sd$. Each hour of each day starting from week 6 onward is overlaid by day. Many cyclical patterns are observable from such overlay as was when looking hourly in \ref{fig:MIT_Hrly}.

\uhoh{Even using 5 weeks, what are we detecting here? Increased communication for those particular 10 min intervals?}

% MIT MT DAILY
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\begin{figure}[H]
\centering
\includegraphics[width=3in,angle=270]{IMG/MIT_3Diff.eps}
\includegraphics[width=3in,angle=270]{IMG/MIT_3Sum.eps}
\caption{$M_t$ of MIT Reality Mining Data overlaid by Day After Week 5. Mean and standard deviation is calculated from first 5 weeks with $\overline{x}$ indicated using a blue solid line and $\overline{x} + 2 sd$ indicated using a mustard yellow dashed line.} 
\label{fig:MIT_Mt}
\end{figure}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

\uhoh{How to apply $M_{it}$ to detect certain individual behaviors, i.e. what thresholds to use? } 

%-----------------------------------------------
%-----------------------------------------------
% conclusions & Future Work
